Quantifying Data Augmentation for LiDAR based 3D Object Detection

In this work, we shed light on different data augmentation techniques commonly used in Light Detection and Ranging (LiDAR) based 3D Object Detection. For the bulk of our experiments, we utilize the well known PointPillars pipeline and the well established KITTI dataset. We investigate a variety of global and local augmentation techniques, where global augmentation techniques are applied to the entire point cloud of a scene and local augmentation techniques are only applied to points belonging to individual objects in the scene. Our findings show that both types of data augmentation can lead to performance increases, but it also turns out, that some augmentation techniques, such as individual object translation, for example, can be counterproductive and can hurt the overall performance. We show that these findings transfer and generalize well to other state of the art 3D Object Detection methods and the challenging STF dataset. On the KITTI dataset we can gain up to 1.5% and on the STF dataset up to 1.7% in 3D mAP on the moderate car class.

==> old_related_work.tex <==
\section{Related Work} \label{related_work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Up until now, most LiDAR based 3D Object Detection methods can be categorized into one out of three categories: \hfill \\
- \textit{Voxel based 3D Object Detection} (section \ref{voxel_based}), \hfill \\
- \textit{Point based 3D Object Detection} (section \ref{point_based}) and \\
- \textit{Voxel \& Point based 3D Object Detection} (section \ref{both_based}). 

In the following subsections, we will give a detailed literature review about these three categories.


\subsection{Voxel based 3D Object Detection} \label{voxel_based} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The earliest works in this line of work include MV3D~\cite{MV3D}, PIXOR~\cite{PIXOR} and AVOD~\cite{AVOD}. They all divide the 3D space into a voxel grid. Then they use hand-crafted features (e.g. point count per voxel) and hand-crafted neighborhood features (e.g. maximum point count per pillar). In the end, they have a 3D Tensor of neighborhood features $(x, y, c)$ and apply regular 2D convolutions on them. The drawback of these methods mostly lies in the hand-crafted feature design.

VoxelNet~\cite{VoxelNet} is one of the seminal works in the area of 3D Object Detection, as a first, this work presents a 3D Object Detection pipeline in an end-to-end fashion without any hand-crafted features. They apply a PointNet-like~\cite{PointNet} architecture to every individual voxel leading to a 4D Tensor $(x, y, z, c)$. Then they perform 3D convolutions to consolidate the $z$-dimension and get a 3D Tensor $(x, y, c')$. Only then they utilize a region proposal network (RPN) based on 2D convolutions.

Another significant contribution to the area of LiDAR based 3D Object Detection is SECOND~\cite{SECOND}, they were able speed up the bottleneck of earlier works, the 3D convolutions, by implementing a sparse 3D convolution layer.

Based on their code-base, PointPillars~\cite{PointPillars} gets entirely rid of the $z$-dimension by only dividing the 3D space into pillars instead of voxels. This change by itself gives a 10-100x speed-up compared to VoxelNet~\cite{VoxelNet}. Additionally, to further speed up the novel encoder, they process each pillar only using a single $1x1$ convolution + max-pooling layer instead of a more complex PointNet-like~\cite{PointNet} architecture. In the end, their final encoder only needs 1.3ms (instead of 190ms in VoxelNet~\cite{VoxelNet}).


\subsection{Point based 3D Object Detection} \label{point_based} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

First, we would like to mention PointNet~\cite{PointNet}. PointNet laid the foundations for many applications, not just for 3D Object Detection. Their work can also be applied to point cloud Classification, Part Segmentation and Semantic Segmentation. The main reason their work is so applicable to multiple domains is because its architecture is relatively lightweight, yet highly efficient and effective, it can process up to one million points per second.

VoteNet~\cite{VoteNet} is a more recent work, that has not proven itself yet on an automotive dataset, but showed promising results on two indoor scene understanding datasets, ScanNet~\cite{ScanNet} and SUN~RGB-D~\cite{SUN}.
VoteNet is an end-to-end 3D Object Detection network based on a synergy of deep point set networks and Hough Voting which does not rely on any kind of anchors.

PointRCNN~\cite{PointRCNN} is another recent work, which also does not need to utilize any anchors. It is a two-stage architecture, where the first stage generates 3D bounding box proposals from a raw point cloud in a bottom-up manner and the second stage refines the 3D bounding box proposals in a canonical representation.


\subsection{Voxel \& Point based 3D Object Detection} \label{both_based} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Both, \textit{voxel} and \textit{point} based 3D Object Detection methods have their strengths and weaknesses. Therefore it only comes naturally that there are methods trying to combine the best of both worlds.

Fast~Point~R-CNN~\cite{FastPointR-CNN} is such a method. It is a two-stage framework, where in the first stage they voxelize the point cloud and feed it to a VoxelRPN to produce a small number of initial predictions. Then, in the second stage, they fuse the features of the box with features from individual points lying inside those proposals and further refine their initial predictions from the first stage.  

Point-Voxel~CNN~\cite{Point-VoxelCNN} is a very recent method that utilizes (coarse) voxels and directly processes the points of the point cloud. Their architecture has two branches, a \textit{low-resolution} voxel based and a \textit{high-resolution} point based branch. The voxel based branch extracts \textit{coarse-grained} neighborhood information, which is supplementary to the \textit{fine-grained} individual point features extracted from the point based branch.
